Improved Knowledge Distillation for Pre-trained Language Models via Knowledge Selection

Knowledge distillation addresses the problem of transferring knowledge from a teacher model to a student model. In this process, we typically have multiple types of knowledge extracted from the teacher model. The problem is to make full use of them to train the student model. Our preliminary study shows that: (1) not all of the knowledge is necessary for learning a good student model, and (2) knowledge distillation can benefit from certain knowledge at different training steps. In response to these, we propose an actor-critic approach to selecting appropriate knowledge to transfer during the process of knowledge distillation. In addition, we offer a refinement of the training algorithm to ease the computational burden. Experimental results on the GLUE datasets show that our method outperforms several strong knowledge distillation baselines significantly.

==> tables/dev_results.tex <==
\begin{table*}[]
	\centering
	\scalebox{0.9}{
	\begin{tabular}{l|ccccccc}
		\toprule[1.1pt]
		Method        & RTE           & MRPC               & MNLI-m/mm & SST-2         & QNLI & QQP       & Avg. \\ \midrule
		BERT\BASESIZE(Teacher) & 71.1 & 90.1/85.5          & 83.7/83.9 & 92.2          & 91.1 & 87.9/91.1 & 85.5     \\ \midrule
		DistilBERT \cite{sanh2019distilbert}    & 59.9          & 87.5/82.4          & 82.2/-    & 91.3          & 89.2 & -/88.5    & -     \\
		w/o KD        &           &           &  &           &  &  &      \\
		Vanilla KD    &           &           &  &           &  &  &      \\ \midrule
		Random-Hard   & 66.3    & 87.3/81.6   &  &           &  &  &      \\
		Random-Soft   & 67.0         & 87.4/81.8          & 82.4/82.7 & 90.4          & 87.2 & 87.4/90.6 & 83.2     \\
		ACKD-Hard (Ours)     & 68.4  & 88.8/83.8          & \textbf{82.6/83.2} & 90.9 & 89.0 & 87.7/90.7 & 84.1     \\
		ACKD-Soft (Ours)    & \textbf{69.0} & \textbf{89.3/84.6} & \textbf{82.6}/82.9 & \textbf{91.5} & \textbf{89.3}     & \textbf{88.0/91.2} &\textbf{84.4}      \\ \bottomrule[1.1pt]
	\end{tabular}
	}
	\caption{
		Results from the GLUE development sets. The best results for each group of student models are in-bold. BERT\BASESIZE is our own implementation of the BERT teacher model. The 6-layer BERT is intended as our student model. For MRPC and QQP, we report F1/Accuracy. We also report the average accuracy for each dataset.
	}
	\label{tab:dev-results}
\end{table*}

==> use-images/fix_kd.tex <==

\begin{table}[]
	\centering
	\scalebox{0.7}{
	\begin{tabular}{lcccc}
		\toprule[1.1pt]
		\multicolumn{1}{c}{\multirow{2}{*}{Knowledge}} & \multicolumn{2}{c}{RTE} & \multicolumn{2}{c}{SST-2} \\ \cline{2-5} 
		\multicolumn{1}{c}{}                           & BERT$_{6}$    & BERT$_{3}$    & BERT$_{6}$     & BERT$_{3}$     \\ \midrule
		FinK                               &65.8&58.1 	&89.7&88.0  \\ \hline
		ResK                               &67.1&56.8   &90.2&87.5  \\ \hline
		FeaK                               &66.1&57.8   &90.4&87.1  \\ \hline
		RelK                               &64.6&58.9   &88.9&88.2  \\ \hline
		FinK\&ResK                         &  &  &  &  \\ \hline
		FinK\&ResK\&FeaK                   &  &  &  &  \\ \hline
		FinK\&ResK\&FeaK\&RelK			   &  &  &  &  \\
		\bottomrule[1.1pt]
	\end{tabular}
}
	\caption{
		Performance of the student models on the development sets from RTE and SST-2 datasets.
		The teacher model is the 12-layer BERT\BASESIZE.
		The student models are the 6-layer BERT$_{6}$ and the 3-layer BERT$_{3}$, respectively.
		Note that the source of knowledge is fixed during the process of KD. 
	}
\end{table}
%\begin{figure}[t!]
%	\centering
%	\includegraphics[scale=0.47]{images/fix_kd.pdf}
%	\caption{
%		Performance of the student models on the development sets from RTE and SST-2 datasets.
%		The teacher model is the 12-layer BERT\BASESIZE.
%		The student models are the 6-layer BERT$_{6}$ and the 3-layer BERT$_{3}$, respectively.
%		Note that the source of knowledge is fixed during the process of knowledge distillation. 
%		}
%	\label{fig:fix-kd}
%	\vspace{-4mm}
%\end{figure}
%%We use the BERT\BASESIZE with 12 layers as the teacher model and use the smaller 6-layer BERT$_{6}$ and 3-layer BERT$_{3}$ as the student model.}

==> use-images/intro_picture.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[scale=0.9]{images/intro_picture.pdf}
	\caption{
		Performance of the student model on the development sets with various categories of knowledge.
		Note that the category of knowledge is fixed during training. }
	\label{fig:fix-kd}
\end{figure}

%We use the BERT\BASESIZE with 12 layers as the teacher model and use the smaller 6-layer BERT$_{6}$ and 3-layer BERT$_{3}$ as the student model.}
